Transformed CNNs: recasting pre-trained convolutional layers with self-attention

Vision Transformers (ViT) have recently emerged as a powerful alternative to convolutional networks (CNNs). Although hybrid models attempt to bridge the gap between these two architectures, the self-attention layers they rely on induce a strong computational bottleneck, especially at large spatial resolutions. In this work, we explore the idea of reducing the time spent training these layers by initializing them as convolutional layers. This enables us to transition smoothly from any pre-trained CNN to its functionally identical hybrid model, called Transformed CNN (T-CNN). With only 50 epochs of fine-tuning, the resulting T-CNNs demonstrate significant performance gains over the CNN (+2.2% top-1 on ImageNet-1k for a ResNet50-RS) as well as substantially improved robustness (+11% top-1 on ImageNet-C). We analyze the representations learnt by the T-CNN, providing deeper insights into the fruitful interplay between convolutions and self-attention. Finally, we experiment initializing the T-CNN from a partially trained CNN, and find that it reaches better performance than the corresponding hybrid model trained from scratch, while reducing training time.

==> checklist.tex <==
\section*{Checklist}
\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{In the conclusion.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNo{Our method, under the conditions examined in the paper, improves robustness while reducing computational costs of training. This is a positive development, however, we acknowledge the fact that robustness is not the only measure that should be tested before deploying AI systems. Therefore, we strongly encourage engineers who utilize any such model to thoroughly test their fairness in the social context in which they plan to deploy their systems.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{Provided in the supplementary material.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See ``Training details'' sections.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNA{The computational cost of the experiments prevented us from using several seeds.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See ``Training details'' sections.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{We use the GPSA layers from~\cite{d2021convit} and evaluate on the robustness datasets ImageNet-C, Imagenet-A and ImageNet-R. In all cases we cited the creators.}
  \item Did you mention the license of the assets?
    \answerNo{ImageNet does not own the copyright of the images but they allow non-commercial downloads of the data under the terms of access laid out in \url{https://www.image-net.org/download}}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNo{In their own words "ImageNet does not own the copyright of the images. ImageNet only compiles an accurate list of web images for each synset of WordNet", this casts doubt on the whether consent has been taken by the creators of the images or not. Unfortunately, IN and variations has become a de facto dataset for benchmarking performance and robustness in CV.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNo{Regarding the ImageNet, we refer the reader to the article ``Excavating AI: The Politics of Images in Machine Learning Training Sets'' by Kate Crawford and Trevor Paglen. It can be reached at \url{https://excavating.ai}}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

==> macros.tex <==
\usepackage{color}
\usepackage{xcolor}
\usepackage{pifont}
\newcommand{\cmark}{\textcolor{green!80!black}{\ding{51}}}
\newcommand{\xmark}{\textcolor{red}{\ding{55}}}

\newif\ifshow
\showtrue
%\showfalse

\ifshow
\newcommand{\ari}[1]{\textcolor{blue}{[\textbf{Ari:} #1]}}
\newcommand{\stephane}[1]{\textcolor{brown}{[\textbf{Stephane:} #1]}}
\newcommand{\levent}[1]{\textcolor{olive}{[\textbf{Levent}: #1]}}
\newcommand{\matthew}[1]{\textcolor{magenta}{[\textbf{Matthew}: #1]}}
\newcommand{\giulio}[1]{\textcolor{cyan}{[\textbf{Giulio}: #1]}}
\newcommand{\hugo}[1]{\textcolor{violet}{[\textbf{Hugo}: #1]}}
\newcommand{\todo}[1]{\textcolor{red}{[\textbf{TODO}: #1]}}
\newcommand{\new}[1]{\textcolor{red}{[\textbf{new}: #1]}}
\else
\newcommand{\ari}[1]{}
\newcommand{\stephane}[1]{}
\newcommand{\levent}[1]{}
\newcommand{\hugo}[1]{}
\newcommand{\matthew}[1]{}
\newcommand{\giulio}[1]{}
\newcommand{\todo}[1]{}
\newcommand{\new}[1]{#1}
\fi


